No More Manual Tests? Evaluating and Improving ChatGPT for Unit Test Generation

Unit testing is essential in detecting bugs in functionally-discrete program units. Manually writing high-quality unit tests is time-consuming and laborious. Although traditional techniques can generate tests with reasonable coverage, they exhibit low readability and cannot be directly adopted by developers. Recent work has shown the large potential of large language models (LLMs) in unit test generation, which can generate more human-like and meaningful test code. ChatGPT, the latest LLM incorporating instruction tuning and reinforcement learning, has performed well in various domains. However, It remains unclear how effective ChatGPT is in unit test generation. In this work, we perform the first empirical study to evaluate ChatGPT's capability of unit test generation. Specifically, we conduct a quantitative analysis and a user study to systematically investigate the quality of its generated tests regarding the correctness, sufficiency, readability, and usability. The tests generated by ChatGPT still suffer from correctness issues, including diverse compilation errors and execution failures. Still, the passing tests generated by ChatGPT resemble manually-written tests by achieving comparable coverage, readability, and even sometimes developers' preference. Our findings indicate that generating unit tests with ChatGPT could be very promising if the correctness of its generated tests could be further improved. Inspired by our findings above, we propose ChatTESTER, a novel ChatGPT-based unit test generation approach, which leverages ChatGPT itself to improve the quality of its generated tests. ChatTESTER incorporates an initial test generator and an iterative test refiner. Our evaluation demonstrates the effectiveness of ChatTESTER by generating 34.3% more compilable tests and 18.7% more tests with correct assertions than the default ChatGPT.

==> tables/dataset_distribution.tex <==

\begin{table}[htb]
	\centering
	\small
	\caption{Benchmark Statistics}\label{tab:datasetDistribution}
	
	\begin{adjustbox}{width=0.5\columnwidth}
	   	
	\begin{tabular}{c|c|c|c}
		\hline
          ~ &  \textbf{Range} & \textbf{Focal Method (\%)} &   \textbf{Test Method (\%)} \\ \hline
          \multirow{4}*{\# Code Lines} & (0,10] & 40.6 &	57.0 \\
            ~ & (10,20]	& 36.8 & 33.2 \\ 
            ~ & (20,30] & 14.0 & 6.4 \\
            ~ & (30, +]     & 8.6 & 3.4 \\
        \hline \hline
        \multirow{4}*{\# Parameters} & [0,1] & 60.0 & - \\
	   ~ & [2,3] & 34.4 & - \\
	   ~ & [4,5] & 4.5 & - \\
	   ~ & [6, +] & 1.1 & - \\
        \hline \hline
        \multirow{4}*{\# Assertions} & [0,2] & -  & 53.1 \\
	       ~ & [3,5] & - & 28.6 \\
	       ~ & [6,8] & - & 10.0 \\
	       ~ & [9, +] & - & 8.3 \\
   \hline
	\end{tabular}
	\end{adjustbox}
 \vspace{-5mm}
\end{table}



==> tables/projectUser.tex <==
\begin{table}[htb]
	\centering
	\small
	\caption{Distribution of Scores for Readability and Usability}\label{table:projectUser}

  \begin{adjustbox}{width=0.7\columnwidth}
\begin{tabular}{
>{\columncolor[HTML]{FE0000}}c 
>{\columncolor[HTML]{FE0000}}c |
>{\columncolor[HTML]{FE0000}}c |
>{\columncolor[HTML]{FE0000}}c |
>{\columncolor[HTML]{FE0000}}c |
>{\columncolor[HTML]{FE0000}}c }
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FE0000}Total Number}                                                                                         & Score & \athenatest{} & \evosuite{} & \ourtool{} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 1     & 494    & 66       & 31         \\ \cline{3-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 2     & 512    & 837      & 426        \\ \cline{3-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \multirow{-3}{*}{\cellcolor[HTML]{FE0000}Naming Intuitiveness}       & 3     & 309    & 412      & 858        \\ \cline{2-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 1     & 484    & 72       & 22         \\ \cline{3-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 2     & 592    & 654      & 406        \\ \cline{3-6} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\cellcolor[HTML]{FE0000}Readability}} & \multirow{-3}{*}{\cellcolor[HTML]{FE0000}Code Structure Rationality} & 3     & 239    & 589      & 887        \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 1     & 545    & 64       & 10         \\ \cline{3-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 2     & 586    & 785      & 528        \\ \cline{3-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \multirow{-3}{*}{\cellcolor[HTML]{FE0000}Semantic Correctness}       & 3     & 184    & 466      & 777        \\ \cline{2-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 1     & 635    & 65       & 20         \\ \cline{3-6} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                              & \cellcolor[HTML]{FE0000}                                             & 2     & 454    & 829      & 347        \\ \cline{3-6} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{\cellcolor[HTML]{FE0000}Usability}}   & \multirow{-3}{*}{\cellcolor[HTML]{FE0000}Reusability}                & 3     & 226    & 421      & 948        \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

